Dissecting Service Mesh Overheads

Service meshes play a central role in the modern application ecosystem by providing an easy and flexible way to connect different services that form a distributed application. However, because of the way they interpose on application traffic, they can substantially increase application latency and resource consumption. We develop a decompositional approach and a tool, called MeshInsight, to systematically characterize the overhead of service meshes and to help developers quantify overhead in deployment scenarios of interest. Using MeshInsight, we confirm that service meshes can have high overhead -- up to 185% higher latency and up to 92% more virtual CPU cores for our benchmark applications -- but the severity is intimately tied to how they are configured and the application workload. The primary contributors to overhead vary based on the configuration too. IPC (inter-process communication) and socket writes dominate when the service mesh operates as a TCP proxy, but protocol parsing dominates when it operates as an HTTP proxy. MeshInsight also enables us to study the end-to-end impact of optimizations to service meshes. We show that not all seemingly-promising optimizations lead to a notable overhead reduction in realistic settings.

==> Makefile <==
###############################################################################
# Project Configuration

TARGET				:= $(shell basename $(PWD)).pdf
MAIN					:= main

#####

TARGET_BASE 	:= $(basename $(TARGET))

################################################################################
# Command Configuration

PDFLATEX			:= pdflatex -shell-escape
BIBTEX				:= bibtex
EPS_TO_PDF		:= epstopdf
OBJ_TO_EPS		:= tgif -print -eps -color -stdout
GNUPLOT				:= gnuplot
SPELLCHECK		:= aspell -c -t --lang=en --personal=$(shell pwd)/ignore.aspell 

################################################################################
# Gathering Information

TEX_MAIN := $(MAIN).tex

TEX_ALL := $(shell search=$(TEX_MAIN); all=; \
				while [ -n "$$search" ] ; do \
					all="$$all $$search"; \
					search=`egrep '^[^%]*\\\\(input|include)' $$search | \
						sed -En 's/.*(input|include)[^\{]*\{(.+)\}.*/\2.tex/p'`; \
				done; \
				echo "$$all")

GFX_ALL := $(shell for t in $(TEX_ALL); do \
				cat $$t | \
				egrep '^[^%]*\\includegraphics' | \
				sed -En 's/.*includegraphics(\[.+\])?\{([^\{]*)\}.*/\2/p'; \
				done)

GFX_FILES := $(shell for g in $(GFX_ALL); do \
					ls $$g.* | \
					egrep "(\.obj|\.eps)$$" | \
					sed -E 's/\.[^ ]+/\.pdf/g'; \
					done)

GNUPLOT_FILES := $(shell for g in $(GFX_ALL); do \
							test -e $$g.p && \
							test ! -e $$g.eps -a ! -e $$g.obj && \
							echo $$g.pdf; \
							done)

BIB_FILES := $(shell cat $(TEX_MAIN) | \
					egrep '^[^%]*\\bibliography\{' | \
					sed -E -e 's/.*\{([^\{]+)\}.*/\1/g' \
						-e 's/([^,\{\}]+)/\1.bib/g' \
						-e 's/,/ /g')	

################################################################################
# Command Rules

all: $(TARGET)

$(TARGET): $(TEX_ALL) $(GFX_FILES) $(GNUPLOT_FILES) $(BIB_FILES)
	$(PDFLATEX) $(TEX_MAIN) </dev/null
	-$(BIBTEX) $(MAIN)
	$(PDFLATEX) $(TEX_MAIN) </dev/null
	$(PDFLATEX) $(TEX_MAIN) </dev/null
	mv $(MAIN).pdf $@

debug:
	@echo "TEX_MAIN = $(TEX_MAIN)"
	@echo "TEX_ALL = $(TEX_ALL)"
	@echo "GFX_ALL = $(GFX_ALL)"
	@echo "GFX_FILES = $(GFX_FILES)"
	@echo "GNUPLOT_FILES = $(GNUPLOT_FILES)"
	@echo "BIB_FILES = $(BIB_FILES)"

clean:
	rm -f $(TARGET) $(TARGET_BASE)-gray.pdf $(TARGET_BASE)-final.pdf \
		*~ *.bbl *.blg *.log *.aux *.toc *.lof *.lot $(MAIN).out $(GFX_FILES) $(GNUPLOT_FILES)

grayscale: $(TARGET_BASE)-gray.pdf

$(TARGET_BASE)-gray.pdf: $(TARGET)
	gs -sOutputFile=$@ -sDEVICE=pdfwrite -sColorConversionStrategy=Gray \
		-dProcessColorModel=/DeviceGray -dNOPAUSE \
		-dBATCH -dAutoRotatePages=/None $(TARGET)

finalized: $(TARGET_BASE)-final.pdf

$(TARGET_BASE)-final.pdf: $(TEX_ALL) $(GFX_FILES) $(GNUPLOT_FILES) $(BIB_FILES)
	$(PDFLATEX) "\\def\\isFinalized{1} \\input{$(TEX_MAIN)}"
	-$(BIBTEX) $(MAIN)
	$(PDFLATEX) "\\def\\isFinalized{1} \\input{$(TEX_MAIN)}"
	$(PDFLATEX) "\\def\\isFinalized{1} \\input{$(TEX_MAIN)}"
	mv $(MAIN).pdf $@

spellcheck: $(TEX_ALL:.tex=.spell)


################################################################################
# File -> File Rules

%.pdf: %.eps
	$(EPS_TO_PDF) $<

%.pdf: %.obj
	$(OBJ_TO_EPS) $< | \
	$(EPS_TO_PDF) -f -o=$@

%.pdf: %.p
	$(GNUPLOT) $< | \
	$(EPS_TO_PDF) -f -o=$@

%.spell: %.tex
	$(SPELLCHECK) $<


